Transformers for Complex Query Answering over Knowledge Hypergraphs

Complex Query Answering (CQA) has been extensively studied in recent years. In order to model data that is closer to real-world distribution, knowledge graphs with different modalities have been introduced. Triple KGs, as the classic KGs composed of entities and relations of arity 2, have limited representation of real-world facts. Real-world data is more sophisticated. While hyper-relational graphs have been introduced, there are limitations in representing relationships of varying arity that contain entities with equal contributions. To address this gap, we sampled new CQA datasets: JF17k-HCQA and M-FB15k-HCQA. Each dataset contains various query types that include logical operations such as projection, negation, conjunction, and disjunction. In order to answer knowledge hypergraph (KHG) existential first-order queries, we propose a two-stage transformer model, the Logical Knowledge Hypergraph Transformer (LKHGT), which consists of a Projection Encoder for atomic projection and a Logical Encoder for complex logical operations. Both encoders are equipped with Type Aware Bias (TAB) for capturing token interactions. Experimental results on CQA datasets show that LKHGT is a state-of-the-art CQA method over KHG and is able to generalize to out-of-distribution query types.

==> original_draft/content.tex <==
\section{Introduction}

Knowledge graphs (KG), as a graph consisting of facts represented by entities as nodes and relations as edges, have attracted much attention in recent years. Triplets (head, relation, tail) are used to represent the binary relational facts in KG. Under Open World Assumption (OWA) \citep{jiSurveyKnowledgeGraphs2022}, most of the currently available is considered incomplete graphs. Both embedding methods and message passing based methods have been proposed to learn the underlying representations of entities and relations in KG, using them to mine undiscovered facts.  \newline

\noindent Complex Query Answering (CQA) in KG has been extensively studied recently and is considered as one of the most important downstream task in Neural Graph Database (NGDB) \citep{renNeuralGraphReasoning2023b}. In the concept of NGDB, KG acts as the data source in graph database, where complex query answering is to perform logical query over incomplete KG via parameterization of entities, relations and logical operators, namely projection, negation, conjunction and disjunction. Different neural query approaches has been proposed to infer the missing links on KG and enriches the answer set with relevant and new answers. For the CQA problem, Existentially quantified First Order queries (EFO-1) is the major type of complex query, which there is one projected variable as the final answer for the query. classic KG representations \citep{trouillonComplexEmbeddingsSimple2016} performed well in one-hop inference, one can iteratively apply KG representations for entity predictions but is insufficient for complex query. In order to answer EFO-1 queries, different approach are proposed to compute the answer sets. Embedding models \citep{chenFuzzyLogicBased2022, renBetaEmbeddingsMultiHop2020, zhangConEConeEmbeddings2021} modeling entities and relations into vector spaces. Then, with query transformed into operators tree format, each logical operators parameterized are used to interact with  with entities embeddings. Other than training embeddings from scratch, approaches like CQD \citep{arakelyanComplexQueryAnswering2021} and LMPNN \citep{wangLogicalMessagePassing2023c} using pretrained KG embeddings are also proposed. These methods utilize KG embeddings that are trained on link prediction task for answering EFO-1 queries. For CQD \citep{arakelyanComplexQueryAnswering2021}, the logical inference step is framed as an optimization problem, where the continuous truth value of an Existential Positive First Order (EPFO) query is maximized by adjusting the variable embeddings. On the other hand, LMPNN \citep{wangLogicalMessagePassing2023c} treated EFO-1 queries as a query graph. Query graph is constructed by entity nodes, variable nodes and relations edges. By instantiating nodes with pretrained KG embeddings, followed by the execustion of message passing to predict the answer embeddings for the EFO-1 query.  \newline

\noindent However, less attention are paid on complex query beyond binary relation. Most of the current models try to tackle CQA problem in ordinary KG focusing only on binary relation. N-ary facts are also abundant in modern large KG. Both Hypergraphs and Hyper-relation graphs are natural choices to construct KG that allows n-ary relations. StarQE \citep{alivanistosQueryEmbeddingHyperrelational2022a} introduces the use of Hyper-relational graph in WD50K-QE, which each triples are constructed from qualified statements (head, relation, tail, qp), where qp are additional qualifier pairs (relation, object) acting as the contextual information for the relation edge. Qualifier pairs can be viewed as the supporting context for the main triples, to distinguish the correct answers from other similar triples. However, Hyper-relational graph are different from Hypergraph in natures. Hyper-relational graph is treating n-ary facts in KG as triples with supporting facts, where triples is the main focus in query answering. There are few models like StarQE \citep{alivanistosQueryEmbeddingHyperrelational2022a} and NQE \citep{luoNQENaryQuery2023b} attempt to solve CQA in n-ary KG under hyper-relational format.\newline

\noindent On the other hand, Hypergraphs is a better choice for representing entities with equal contribution in the relation involved. For example, for relation\textit{ coauthor(authorA,authorB,authorC)}, it can be correctly represented by hyperedge in hypergrpah but incorrectly represented as coauthor(authorA,authorC, (coauthor,authorB)) in hyper-relational graph, where authorB is a supporting statements for coauthor(A,C). In facts, there are efforts been put in constructing Knowledge Hypergraphs Embeddings for Knowledge Hypergraphs (KHG) like M-FB15k \cite{fatemiKnowledgeHypergraphsPrediction2020a} and JF17k  \citep{wenRepresentationEmbeddingKnowledge2016a}, which all are trained for link prediction. There are little effort has been put in CQA in KHG. LSGT (citation) is the only work that investigated CQA involved ordered hyperedges, where hyperedges act as the starting facts for multi-hop inference. However, for subsequent hops, it uses the binary relation for intermediate variable nodes in predicting the answers. We are aware that there are no experiment for CQA in KHG under full n-ary multi-hop inference settings, has been conducted yet.\newline

\noindent In this paper, we propose a novel 2-stage transformer models, \textbf{L}ogical \textbf{K}nowledge \textbf{H}yper\textbf{g}raph \textbf{T}ransformer \textbf{(LKHGT)}, a transformer-based approach to perform reasoning over KHGs, which is capable of generalizing CQA problem from binary relation to n arity relations. LKHGT consist of 2 encoder which are Projection Encoder and Logical Encoder. Inspired by Heterogenous Graph Attention Network \citep{wangHeterogeneousGraphAttention2021}, both Projection Encoder and Logical Encoder adopt inductive bias for different token types to conform with the token type heterogeneity. Projection Encoder is responsible for predicting answers for variables in atomic hyperedge, while Logical Encoder is responsible for deriving the intermediate variable embeddings for each type of logical operations.
We first define the logical query in the form of EFO-1 Disjunctive Normal Form and constructed ordered query hypergraphs accordingly. In the query graph, every ordered hyperedge represents an atomic formula that includes a predicate potentially accompanied by a negation operator. Then we will investigate the performance of LKHGT with other baselines models. For each one-hop atomic formula, we utilize the pretrained knowledge hypergraph representation to derive intermediate embeddings based on the neighboring entity embedding, relation embedding, direction information, and negation details. To conduct fair experiment, we included multiple methods that is capable to reason on hypergraphs and we also extended the framework of LMPNN \citep{wangLogicalMessagePassing2023c} to relational ordered knowledge hypergraphs, utilizing pretrained KHG embeddings with logical inference capabilities from Hypergraph Message Passing Networks. we extended the sampling rationale for binary relation cqa \citep{wangLogicalMessagePassing2023c} to n-ary ordered hyperedge format, and created a new relational ordered hypergraphs CQA dataset, JF17k-HCQA and M-FB15k-HCQA. \newline

\noindent Our experiments shows that, LKHGT outperform others N-ary CQA models in the ordered hyperedge settings. We show that our models can generalize from edges of arity 2 to arity N and obtains promising results. Due to the framework's nature, after encoder learning basic logical operations, our models also shown good result in out of distribution queries. Through the comparison of using Logical Encoder and Fuzzy logic \citep{zadehFuzzyLogic1988} in performing logical operations, we also shows that using Transformer based encoder outperform neural symbolic methods utilizing fuzzy logic operation. Hence, our approach is the first to bridges the gap between Complex Query Answering and Knowledge Hypergraph.

\section{Related Works}

\subsection{Knowledge Hypergraphs Embedding}
BoxE \citep{abboudBoxEBoxEmbedding2020}, HypE, ReAlE \citep{fatemiKnowledgeHypergraphEmbedding2021a, fatemiKnowledgeHypergraphsPrediction2020a}, n-Tucker \citep{liuGeneralizingTensorDecomposition2020a}, m-TransH \citep{wenRepresentationEmbeddingKnowledge2016a} and RAE \citep{zhangScalableInstanceReconstruction2018} are Knowledge Hypergraphs Embeddings that considered n-ary facts in the form of r(e1, e2 . . .). These methods aims to perform link prediction by encoding entities and relations into embeddings continuous spaces. These models are equivalently performing projection on atomic hyperedge. Although they can perform well in atomic query projection task, they lack the ability to perform multi-hop query, where performance degrades as projection continues on sub-queries. To enable logical operations on these embeddings, fuzzy logic \citep{zadehFuzzyLogic1988, chenFuzzyLogicBased2022} or message passing methods \citep{wangLogicalMessagePassing2023c} can be applied.

\subsection{N-ary graph Message Passing}
N-ary graph message passing is related and is one of the important ingredients in constructing models for higher order knowledge graph CQA. Most of the previous works focus in hypergraph message passing \citep{agarwalHigherOrderLearning2006, yadatiHyperGCNNewMethod2019, yadatiNeuralMessagePassing2020a}, while some of them are tailored for hyper-reltaional graphs. StarE \citep{galkinMessagePassingHyperRelational2020}, GRAN \citep{wangLinkPredictionNary2021}, are the attempts to solve one hop query on hyper relational KG. For knowledge hypergraphs,
HR-MPNN \citep{huangLinkPredictionRelational2024a}, G-MPNN \citep{yadatiHyperGCNNewMethod2019}, RD-MPNN \citep{zhouDynamicRelationLearning2023}, are approaches that utilize Message Passing Networks in Hypergraphs. G-MPNN \citep{yadatiHyperGCNNewMethod2019} is the first message passing network tailored for relational hypergraphs, while RD-MPNN \citep{zhouDynamicRelationLearning2023} further improve G-MPNN by incoporating positional information for entities in hyperedges. HR-MPNN \citep{huangLinkPredictionRelational2024a} formally defined the first General Relational Ordered Hypergraphs Message Passing Framework and proposed HCNet for inductive settings. In ther ordered Utilizing the idea from LMPNN \citep{wangLogicalMessagePassing2023c}, one of our baseline combined HR-MPNN \citep{huangLinkPredictionRelational2024a} with pretrained embeddings. 

\subsection{Complex Query Answering}
For ordinary CQA, there are multiple approaches, including transformer, query embeddings, neural-symbolic, message passing methods. After the introduction of LMPNN \citep{wangLogicalMessagePassing2023c}, different pretrained KG embeddings can be easily utilized in the task of CQA, pretrained embedding can act as the the initial entities and relations embeddings. One can obtain the final answers embeddings through message passing on query graphs. These embeddings include RESCAL \citep{nickelThreewayModelCollective2011}, TransE \citep{bordesTranslatingEmbeddingsModeling2013}, DistMult, ComplEx \citep{trouillonComplexEmbeddingsSimple2016}, ConvE, RotatE. GNN-QE \citep{zhuNeuralSymbolicModelsLogical2022}. 
For query embeddings approach, GQE \citep{hamiltonEmbeddingLogicalQueries2019a} is the query embeddings model for solving queries involved existential quantifiers and conjunction. FuzzQE \citep{chenFuzzyLogicBased2022} furtherly use fuzzy logic to define logical operators. 
\noindent For neural-symoblic approach, various methods like BetaE \citep{renBetaEmbeddingsMultiHop2020}, ConE \citep{zhangConEConeEmbeddings2021} and QUERY2BOX \citep{renQuery2boxReasoningKnowledge2020} uses different embedding methods to project symbol to continuous space for query answering. MLPMix \citep{amayuelasNeuralMethodsLogical2022} and NewLook \citep{liuNeuralAnsweringLogicalQueries2021} uses MLP and MLP with attention for CQA problems.  ENeSy \citep{xuNeuralSymbolicEntangledFramework2022},  QTO \citep{baiAnsweringComplexLogical2023}and CQD \citep{arakelyanComplexQueryAnswering2021} utilize combinatorial optimization on query computation tree and complex query itself for query answering.
\noindent Prevuous studies on complex query answering mainly expanded on knowledge graphs. Extensive studies has been conducted on ordinary knowledge graph to deal with OWA by using existing triples in KG to generalize to predict unseen triples. Most Studies has shown promising performance in large scale knowledge graph. EFO-1 Query can be answered in an effective and efficient manner given the arity is equals to 2. 
However, most of the studies cannot naturally extend their methods to general n-ary facts in either hyperedge or hyper-relational format.


\subsection{Transformer in CQA}
Since the introduction of Transformer \citep{vaswaniAttentionAllYou2023b}, there has been several attempts to adopt transformer for solving CQA problem. SQE \citep{baiSequentialQueryEncoding2023} transformed EFO-1 queries into linearized computational graph and feed it into sequence encoder. QTP \citep{xuQuery2TripleUnifiedQuery2023} separate simple and complex query, training neural link predictor and query encoder for each query type respectively. Query Encoder responsible for projecting each token into continuous space. Neural link predictor perform embedding estimation using projected embeddings. Besides, there are also extensive research focusing on inductive bias, for example, relative positional encoding \citep{shawSelfAttentionRelativePosition2018} that capture relative position of input tokens. Rotary embedding \citep{suRoFormerEnhancedTransformer2023} capturing both absolute and relative position information by rotating position information vector. Each position encoding methods acts as the inductive bias for self-attention in Transformer. HAN \citep{wangHeterogeneousGraphAttention2021} introduces transformer based methods in solving link prediction on knowledge graph, where distinct bias are trained for different meta paths. KnowFormer (cite knowformer) is a knowledge graph transformer with inductive bias for each specific relation type performing simple query answering. TEGA \citep{zhengEnhancingTransformersGeneralizable2025} propose to use inductive bias according to token types interaction and have EFO-syntax query as input for CQA problem. 

\subsection{N-ary Graph Reasoning}
First N-ary reasoning problem introduced in the field of CQA is performed on hyper-relational knowledge graph. TransEQ \citep{liuGeneralizingHyperedgeExpansion2024} is an query embedding models that generalize star expansion (cite higher order learning) for hyper-edges to hyper-relational graphs, then use encoder-decoder to capture structural information and semantic information for hyper-relational knowledge graph completion task. NeuInfer \citep{guanNeuInferKnowledgeInference2020} chose to represent n-ary fact as a primary triple coupled with a set of its auxiliary descriptive attribute-value pair(s) and use neural network to perform knowledge inference.
StarQE \citep{alivanistosQueryEmbeddingHyperrelational2022a} utilize StarE \citep{galkinMessagePassingHyperRelational2020} as graph encoder for StarQE, equip it with message passing to have the ability to deal with multi-hop queries. NQE \citep{luoNQENaryQuery2023b} use dual-heterogeneous Transformer encoder and fuzzy logic \citep{zadehFuzzyLogic1988} to recursively process hyper-relational query tree. However, hyper-relational edges encode entities with possibly different relation in a single triples, which does not exhibit same characteristics as hyperedges. The encoder input format for NQE generalize n-ary inputs, thus it can be naturally extend to be used in hyper-edges query answering.
SessionCQA \citep{baiUnderstandingInterSessionIntentions2024}, The first CQA model incorporates the concept of hyper-edges, encoding user sessions as hyper-edges for item recommendations. However, its query type does not follow a fully hyper-edge setting; only the initial first hop is represented as a hyper-edge, while subsequent hops use binary relation edges.
The query input format for SessionCQA can also naturally extend for N-ary facts.


\section{PRELIMINARIES}
\subsection{Knowledge Hypergraphs}
\begin{definition} A knowledge hypergraph $ \mathcal{G} = (\entities, \relations, \hyperedges)$, where $\entities$ is the set of entities $e$ in knowledge hypergraph. $\relations$ is the set of relation $r$. $\hyperedges$ is the set of ordered hyperedges $h = r(e_1,...,e_k) \in \hyperedges$, where $e_1, .., e_k \in \entities$ and $r \in \relations$. Arity of a hyperedge $h$ is defined as $k = ar(r)$, where each relation type comes with fixed arity size. Each atomic query $\textbf{a}$ is $\in \hyperedges$.
\end{definition}
\noindent Although  through star expansion \citep{agarwalHigherOrderLearning2006} of hyperedge, an hyperedge can be converted to homogeneous graph, however structural information will be loss in process.
\begin{figure}
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=.5\linewidth]{fig/operator_tree.png}
  \caption{Operator Tree}
  \label{fig:tree}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=.5\linewidth]{fig/query_graph.png}
  \caption{Hyperedge Query Graph}
  \label{fig:graph}
\end{minipage}

\end{figure}
\subsection{EFO-1 Query in Hypergraphs}
In this paper, we will focus on Existential First Order queries with a single free variable with logical formulas (EFO-1) under the disjunctive normal form. \newline

\noindent An atomic formula $a$ is composed of term, relation and variable. A simplest atomic formula can be intuitively represented by an ordered hyperedge $h = r_1(e_1,...,v_k)$, where $e_1$ is a term, $v_k$ is an variable at position k and $r_1$ is the relation. Let $ar(r)$ is the arity of the given relation $r$. A knowledge graph is a relational knowledge hypergraph where for all $r \in \mathcal{R}, ar(r) = 2$. An atomic formula can be negated by adding $\neg$ to form $\neg r(e_1,...,v_k)$. A first order formula can be iteratively constructed by atomic formula $a$ using connectives conjunction $\land$ and disjunction $\lor$. Quantifiers can be added to variables in $a$ using quantifiers like $\exists$ and $\forall$. Variables without quantifiers is considered as free.

\begin{definition}
Given a knowledge hypergraph $\mathcal{G}$, an EFO-1 query $q$ is defined as a first-order formula in the below DNF form, 
\end{definition}
\begin{equation}
q(y,x_1,...,x_n) =  \exists x_1, \ldots, \exists x_m [ (a_{11} \land a_{12} \land \cdots \land a_{1n_1}) \lor \cdots \lor (a_{p1} \land a_{p2} \land \cdots \land a_{pn_p}) ]
\end{equation}
where y is the only free variable, and $x_i$ for $1 \leq i \leq m$ are existential variables. Each brackets represent an complex query where each $a_{ij}$ is an atomic formula with constants $y,x_i$ and variables that can be either negated or not.
To address the EFO-1 queries, one must determine the answer set A[$Q,KG$]  such that for each a $\in$ A[$Q,KG$], $q(y=a, x_1,...,x_n)$ returns true. \newline



\noindent Considering a query in the form of $r_1(e_1,..,v_1) \land r_2(e_1,e_2,v_1) \land r_3(v_1,e_3,f_1)$, there are 2 ways to represent EFO-1 queries in hypergraphs, which are query graphs and operator tree.
\newline
\noindent \textbf{Operator tree} In operator tree, each node itself is an operator node that corresponds to logical operations like, projection, conjunction, disjunction, negation. In knowledge hypergraph settings, each projection node consists of set of entities for itself and a variable nodes in random arity position. As Figure \ref{fig:tree} shown, $r_1$ and $r_2$ are presented by the 2 projection nodes. Each of the two projection node is pointed to the intersection node, and the intersection node represent the conjunction of answer sets from its pointers. Intersection node pointing to last projection node representing $r_3$, which use the intersected variable and remaining set of entities to obtain the final answer after projection.
\newline 
\noindent \textbf{Query graph} In Figure \ref{fig:graph}, each hyper edge representing an atomic formula containing edge information like relation types and negation information. The nodes involved are either constant symbol, free variable or existential variable. \newline

\noindent In this paper, each Knowledge Hypergraph EFO-1 query is presented in the form operator tree for LKHGT. As we can see that in order to allow transformer to perform message passing alike operation through the self-attention mechanism, we have to encode whole query in a single pass. When transformer based model encode whole query graphs as a sequence of tokens, it becomes more challenging for transformers to focus on solving each atomic query in the multihop-query. Thus, operator tree is more suitable for our choice of modeling.



\section{Logical Knowledge Hyper Graph Transformer}
\begin{wrapfigure}{r}{0.4\textwidth}  % 'r' for right, 'l' for left
    \centering
    \includegraphics[width=0.4\textwidth]{fig/example.png}  % Replace with your image
    \caption{Example of LKHGT processing query tree}
    \label{fig:example}
\end{wrapfigure}
In this section, we will describe the how operator tree is used to represent complex query, and explain how the 2 stage encoder, Logical Knowledge Hyper Graph Transformer, works given a query tree input. In order to allow precise estimation of answer set, we propose to use 2 stage encoder to process the query tree iteratively. For example, refer to Figure \ref{fig:example}, we can see that each projection node at bottom level first receive necessary information like, negation, relation, entities and position of variable node inside the hyperedge. Then these information is fed into projection encoder for each projection. Intersection is then performed with logical encoder, which is done by receive all variable embeddings output from each projection encoder. Finally, projection perform last projection using the answer set embeddings output from projection encoder. Although using iterative method to process query tree is slower comparing to encoding whole query graph at once, we ensure the correctness of answer set embeddings output for each atomic formula.
\subsection{Tokens Input and Output}
Operators type included in operator tree are projection (p), negation ($\neg$), intersection ($\land$), union ($\lor$). As defined, each complex query is composed of atomic formula which is made of relaiton (r), subject (s), variable (e). Overally speaking, there are 7 types of token. Relation, subject, variable and negation type of tokens will be fed into projection encoder. Projection, intersection, union types of token will be fed into logical encoder.

\noindent\textbf{Projection Encoder} Given the fact that negation can only applied to atomic formula which is represented as projection operation, we chose to process negation operation in projection encoder. Projection Encoder projects tokens into continuous space according to their token type. If negation is involved, the input tokens will be, 
\begin{equation}
    tokens = T_p = [n,r_1,s_1,e_2,...] 
\end{equation}
The corresponding projected sequence will be,
\begin{equation}
    X = W_pT_p = [W_nx_1,W_rr_1,W_ss_1,W_ee_2,...] \in R^{n \times d}
\end{equation}
where $W_{p} \in R^{d \times d} , p \in \{ n, r, s, e\} $ is the linear projection weight.  \newline 
Since projection encoder is performing projection ordered hyperedge, we will also add absolute positional encoding to entities node and variable node, let the set of nodes be $N$ for an hyperedge, then the input embeddings will be.
\begin{equation}
    X_{v\in N} = X_{v\in N} + PE_{pos}
\end{equation}
\noindent\textbf{Logical Encoder}
Logical encoder will focus in dealing with logical task that involves more than 1 projection node, which is intersection (conjunction) and union (disjunction). These nodes will receive pointers from more than one operators node, we use transformer logical encoder to encode all projected variable, the input tokens for logical encoder will be,
\begin{equation}
    tokens = T_l = [i/u,p_1,p_2,p_3,...] 
\end{equation}
The corresponding projected sequence will be,
\begin{equation}
    X = W_lT_l = [W_{i/u} \{i/u\},W_pp_1,W_pp_1,W_pp_2,...] \in R^{n \times d}
\end{equation}
where $W_{l} \in R^{d \times d} , l \in \{ i, u, p\} $ is the linear projection weight. 
Both projected sequence is then further process with modified version of \citep{vaswaniAttentionAllYou2023b}. Finally, Projection Encoder will output embeddings of variable node in hyperedge and Logical Encoder will output the embeddings of the logical operator tokens.
\newline
\noindent 
\begin{figure}
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=0.75\linewidth]{fig/PE.png}
  \caption{Projection Enconder}
  \label{fig:pe}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=0.75\linewidth]{fig/LE.png}
  \caption{Logical Encoder}
  \label{fig:le}
\end{minipage}

\end{figure}

\subsection{Guided attention for Projection Encoder and Logical Encoder}

Inspired by the idea of introducing inductive bias for meta paths in \citep{wangHeterogeneousGraphAttention2021}, LHKGT also introduced modified inductive bias tailored for CQA task. With the given 7 token types, we can observe there are types of token interaction bias to be added into self attention matrix. For Projection Encoder there are $P^4_2$ edge types for token types [$n,r,e,v$]. For Logical Encoder, there are $P^3_2$ edge types for token types. In order to cater for these edge types differences, we construct the attention matrix with inductive bias as below: 
\begin{equation}
    e_{ij} = \frac{x_i W^Q_o(x_j W^k_o + B^K_{ij})^T}{\sqrt{d}} , a_{ij} = softmax(e_{ij})
\end{equation}
\begin{equation}
    z_i = \sum^n_{j=1} a_{ij}(x_j W^V_o + B^V_{ij})
\end{equation}
Where $B_{ij}$ is the guided attention for token interaction, ($W^Q,W^K,W^V$) is the linear projection matrix $\in R^{d\times d}$ and $\{ o, i, j\}$ can be the seven token types $\in \{n,r,e,s,p,i,u\}$. These bias able to differentiate the token types interaction and help facilitates the capture of nuanced interactions among token types, allowing the transformer to adaptively weigh the importance of each token based on its role in the context. 

\noindent In our case, we can treat Transformer is a special case of GNN. For Projection encoder, each edge is an fully connected graph input in the perspective of GNN. We are doing aggregation with attention on this fully connected graph and predict the embeddings of the projection node using transformer self-attention mechanism. This aggregation process not only enriches the embeddings of the projection node but also ensures that the model can dynamically adjust to the significance of different tokens based on the context. The result is a robust embedding that encapsulates the rich relational structure inherent in the input data.

\subsection{Transformer as the replacement for Fuzzy Logic}
Most of the current CQA models utilize fuzzy logic as their key component in determining the answer set. These models share an assumption that the embeddings of final answers is the representation of a single entity in the knowledge graph. Logical encoder output a continuous space representation of answer set.

\subsection{Training LKHGT}
After obtaining the output embeddings $f \in R^{d}$, we can compute the output label of the entity by a simple MLP decoder and have output $\hat{y} \in R^{|\mathcal{E}|}$. Given a the query embedding $\hat{y}$, we can first use a softmax function to obtain the probability scores of query embedding between all entity,
\begin{equation}
    \sigma (\hat{y}) = \frac{e^{\hat{y}_i}}{\sum_j e^{\hat{y}_j}}
\end{equation}
Then we can construct the cross-entropy loss to maximize the log probability of $\hat{y}$ matching the answer $a$,
\begin{equation}
    L = - \frac{1}{N} \sum_i log (\sigma(\hat{y}))
\end{equation}
where N is the batch size.

\section{Experiments}
In this section, we will describe the experiment set up including dataset, baselines and evaluation methods.


\subsection{Dataset}
Since Knowledge Hypergraph CQA is a subfield of CQA problem that has not been investigated before, thus we created custom Dataset JF17k-HCQA and M-FB15k-HCQA. Following the rationale from binary CQA sampling methods(Wang et al., 2021), we modified the sampling methods into hypergraph version (Appendix \ref{sec:appendixC}), created datasets consists of query types (1P 2P 3P 2I 3I PI IP 2U UP 2IN 3IN INP PIN PNI), total 14 types, including all logical operation. 

\subsection{Baselines}
For baseline models, we chose NQE \citep{luoNQENaryQuery2023b} and LSGT \citep{baiUnderstandingInterSessionIntentions2024} as our baseline modes. NQE is a method that encode hyper-relational facts from KG into embeddings. LSGT encode query graph information like, nodes ids, graph structure and logical structure using a bert transformer (cite).As NQE \citep{luoNQENaryQuery2023b} uses hyper-relational edges as input for its encoder. So, we followed the implementation of NQE in \citep{baiUnderstandingInterSessionIntentions2024} and modified our data format to feed it into NQE. For LSGT, we transformed our data into unified id format for input. For fair comparison, we replace all models encoder with simple basic transformer layer without modifying the other implementation details. Transformer embedding size is set to be 400 for iterative model like NQE and LKHGT. For LSGT, its embedding size is set to be 1024 in order to have it converge.
Aside from transformer based model, we also implemented HLMPNN (Appendix \ref{sec:appendixA}), a hypergraph version of LMPNN \citep{wangLogicalMessagePassing2023c}, which is set to have embedding size of 200. All models are trained on 1 3090 GPU with 400 epochs.
\subsection{Evaluation}
In all experiments, we follow the common practice, sampled query from Knowledge Hypergrpahs $\mathcal{G}_{train}, \mathcal{G}_{val}, \mathcal{G}_{test}$, where $\mathcal{E}_{train} \subset \mathcal{E}_{val}$ and $\mathcal{E}_{val} \subset \mathcal{E}_{test}$. We select the mean reciprocal rank (MRR) defined as,
\begin{equation}
    MRR(q) = \frac{1}{||v||}\sum_{v_i \in v} \frac{1}{rank(v_i)}
\end{equation}
as the evaluation metric to evaluate the ranking. For each query instance, we initially rank all entities, excluding those identified as easy answers, by their cosine similarity to the query variable embedding. The rankings of the hard answers are then used to calculate the Mean Reciprocal Rank (MRR) for that particular query instance. Finally, we compute the average of the metrics across all query instances. In this paper, we report and compare the MRR results.

\subsection{Results}
Table 1 presents the MRR results of LKHGT and other baseline models for answering EFO-1 queries across the two CQA datasets. It demonstrates that LKHGT achieves state-of-the-art performance on average for both EPFO and negation queries. When comparing LKHGT with transformer-based and message-passing methods, we observe that the message-passing methods significantly underperform. Additionally, when comparing the Iterative Model (LKHGT \& NQE) to the Sequential Model (LSGT), the Iterative Model shows superior performance. This advantage may be attributed to their approach of encoding the entire query at once, which can hinder performance on complex queries. In contrast, the LKHGT model shows notable improvements, particularly when replacing fuzzy logic with a logical encoder in the NQE framework, enhancing its ability to handle conjunctions and disjunctions effectively. Interestingly, LKHGT outperforms NQE on negation queries, despite incorporating negation in the Projection Encoder rather than relying on fuzzy logic. This suggests that fuzzy logic may not be sufficient for addressing complex query-answering tasks. Overall, these findings confirm that the two-stage architecture of LKHGT successfully enhances performance in complex query scenarios, demonstrating its effectiveness and robustness in the context of query answering.
\begin{center}
\begin{table}
\scriptsize
\caption{MRR results of different CQA models on two KHGs. AP represents the average score of
EFO-1 queries and AN represents the average score of queries with negation. The boldface indicates
the best results for each KG.}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{llllllllllllllllll} \toprule
KHG & Model & 1P & 2P & 3P & 2I & 3I & PI & IP & 2U & UP & 2IN & 3IN & INP & PIN & PNI & AP & AN \\ \midrule
\multirow{ 2}{*}{JF17k}  
 & HLMPNN & 45.26 &  7.26 & 13.38 & 46.08 & 48.36 & 16.01 &  8.54 & 24.99 & 13.28 & 10.35 & 15.49 & 11.48 &  7.32 &  8.24 &      24.80 &     10.58 \\
 & LSGT & 50.56 & 21.85 & 17.75 & 53.34 & 53.71 & 32.06 & 20.78 & 22.49 & 18.33 & 14.00 & 16.40 &  6.05 &  7.44 &  8.59 &      32.32 &     10.50 \\ 
 & NQE &  56.37 & 39.18 & 39.21 & 65.41 & 72.37 & 55.36 & 39.22 & 29.05 & 39.36 & 21.68 & 28.83 & 20.25 & 16.21 & 22.13 &      48.39 &     21.82 \\ 
 & LKHGT & 58.43 & 43.89 & 42.75 & 69.11 & 75.19 & 58.19 & 43.16 & 32.05 & 42.51 & 26.26 & 31.62 & 23.18 & 18.74 & 25.35 &      51.70 &     25.03  \\ 

 \hline
\multirow{ 2}{*}{M-FB15k}  
 & HLMPNN & 44.62 &  7.24 & 13.45 & 46.03 & 48.63 & 16.35 &  8.61 & 25.03 & 13.51 & 10.84 & 15.82 & 11.41 &  7.35 &  8.45 &      24.83 &     10.77 \\
 & LSGT & 40.31 & 21.72 & 17.03 & 29.26 & 33.51 & 23.03 & 19.43 & 13.11 & 19.20 & 12.48 & 15.76 & 18.77 &  7.45 & 13.34 &      24.07 &     13.56 \\ 
 & NQE & 48.07 & 34.42 & 31.15 & 46.63 & 56.97 & 36.03 & 32.15 & 17.41 & 30.43 & 22.99 & 32.45 & 28.17 & 18.05 & 24.22 &      37.03 &     25.17 \\ 
 & LKHGT & 3 & \\ 
   
\bottomrule
\end{tabular}}
\end{table}
\end{center}


\subsection{Ablation Study}
\noindent In the ablation study, we conduct further experiments to justify the effects of the logical encoder and the positional encoding of LKHGT. All experiments are performed on queries over JF17k. We also include an experiment to test the out-of-distribution generalization of our models by training them with minimal queries that involve all logical operations, specifically (1p, 2i, pi, 2in, pin, 2u). Table 2 presents the results of the ablation study. From the results, we observe that without the positional encoding, the model's performance degrades, indicating the importance of this bias for identifying the position of each nodes to enhance performance. When using LKHGT with fuzzy logic, the results are similar to those of NQE, suggesting that the transformer-based logical encoder is a key component in improving performance.
\newline
\noindent In the out-of-distribution (OOD) settings, we find that while queries can generalize, such as $pin$ and $pni$, the interaction bias is learned. However, for instances like $2u$ and $up$, the interaction bias between 
$u$ and $p$ is not observed during the training stage, resulting in a lack of generalization. This highlights that the model's weakness lies in its ability to train on all possible types of interactions between token types.

\noindent \textbf{Operator Cardinality}
\begin{center}
\begin{table}
\scriptsize
\caption{MRR results of LKHGT in fuzzy settings, absolute position encoding and OOD setting.}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{llllllllllllllllll} \toprule
KHG & Model & 1P & 2P & 3P & 2I & 3I & PI & IP & 2U & UP & 2IN & 3IN & INP & PIN & PNI & AP & AN \\ \midrule
\multirow{ 2}{*}{JF17k}  
 & LKHGT & 55.49 & 40.57 & 40.58 & 67.35 & 72.64 & 56.31 & 40.37 & 30.59 & 40.92 & 24.54 & 30.03 & 22.31 & 18.07 & 23.89 &      49.43 &     23.77  \\ 
  & LKHGT w/ fuzzy. & 55.49 & 40.57 & 40.58 & 67.35 & 72.64 & 56.31 & 40.37 & 30.59 & 40.92 & 24.54 & 30.03 & 22.31 & 18.07 & 23.89 &      49.43 &     23.77  \\ 
 & LKHGT w/o abs. & 57.12 & 42.58 & 41.95 & 68.56 & 73.60 & 57.03 & 41.92 & 31.31 & 41.91 & 25.70 & 31.52 & 22.82 & 18.14 & 24.56 &      50.66 &     24.55  \\ 
 & LKHGT w/ ood. cardinality = 3 & 54.44 & 21.33 & 17.73 & 64.20 & 39.90 & 52.21 & 21.24 & 29.25 & 21.65 & 24.71 & 16.44 & 11.96 & 16.42 & 22.04 &      35.77 &     18.31  \\ 
  & LKHGT w/ ood. cardinality = 2 & 54.44 & 21.33 & 17.73 & 64.20 & 39.90 & 52.21 & 21.24 & 29.25 & 21.65 & 24.71 & 16.44 & 11.96 & 16.42 & 22.04 &      35.77 &     18.31  \\ 
   
\bottomrule
\end{tabular}}
\end{table}
\end{center}

\section{Conclusion}
In this paper, we present the Knowledge Hypergraph CQA dataset to bridge the current gap in complex question answering (CQA) within hypergraph settings. We propose LKHGT to answer complex queries over Knowledge Hypergraphs, particularly EFO-1 queries. LKHGT achieves strong performance through its two-stage architecture, which incorporates both a Projection Encoder and a Logical Encoder. In the ablation study, we demonstrate that the use of inductive bias further enhances performance. Our research effectively addresses the gap in EFO-1 query answering tasks in hypergraph settings while highlighting the limitations of fuzzy logic. The experiments show that, given sufficient training on various query types, LKHGT is the state-of-the-art model for current CQA tasks involving Knowledge Hypergraphs.

difference in query types for training set and test set.

==> original_draft/custom_command.tex <==
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem*{remark}{Remark}
\newtheorem{proposition}{Proposition}
\newtheorem{conjecture}{Conjecture}
\newtheorem{question}{Question} 
\newtheorem{definition}{Definition}

\newcommand{\re}{\mathrm{Re}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\V}{{\rm Var}}

\newcommand{\lang}{\mathcal{L}}
\newcommand{\kg}{\mathcal{KG}}
\newcommand{\khg}{\mathcal{KHG}}
\newcommand{\entities}{\mathcal{E}}
\newcommand{\relations}{\mathcal{R}}
\newcommand{\hyperedges}{\mathcal{H}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
